StreamOptix: A Cross-layer Adaptive Video Delivery Scheme

This paper presents a cross-layer video delivery scheme, StreamOptix, and proposes a joint optimization algorithm for video delivery that leverages the characteristics of the physical (PHY), medium access control (MAC), and application (APP) layers. Most existing methods for optimizing video transmission over different layers were developed individually. Realizing a cross-layer design has always been a significant challenge, mainly due to the complex interactions and mismatches in timescales between layers, as well as the presence of distinct objectives in different layers. To address these complications, we take a divide-and-conquer approach and break down the formulated cross-layer optimization problem for video delivery into three sub-problems. We then propose a three-stage closedloop optimization framework, which consists of 1) an adaptive bitrate (ABR) strategy based on the link capacity information from PHY, 2) a video-aware resource allocation scheme accounting for the APP bitrate constraint, and 3) a link adaptation technique utilizing the soft acknowledgment feedback (soft-ACK). The proposed framework also supports the collections of the distorted bitstreams transmitted across the link. This allows a more reasonable assessment of video quality compared to many existing ABR methods that simply neglect the distortions occurring in the PHY layer. Experiments conducted under various network settings demonstrate the effectiveness and superiority of the new cross-layer optimization strategy. A byproduct of this study is the development of more comprehensive performance metrics on video delivery, which lays down the foundation for extending our system to multimodal communications in the future. Code for reproducing the experimental results is available at https://github.com/Evan-sudo/StreamOptix.

==> draft.tex <==
\subsection{MAC: Video-aware Resource Allocation}
The MAC layer efficiently employs a scheduler to manage the allocation of RBs. As previously discussed, both the MCS and RB allocation influence the TB size, thereby adjusting the link's throughput. However, the MCS is controlled by link adaptation, which needs to strictly adhere to the BLER constraint. Increasing the MCS inherently increases the risks of block errors, potentially decreasing the final throughput. Hence, we modify the RB allocation strategy at MAC to align the throughput more closely with chunk bitrate. It is important to note that the bitrate ladder in rate adaptation has significant gaps between adjacent bitrates. Furthermore, throughput prediction can be unreliable. Adjustments to the throughput are frequently necessary to match with the chosen bitrate.
As the chunk length (order of seconds) are much longer compared to TTIs (order of milliseconds) for resource allocation, it is challenging for MAC to quickly impact the bitrate decisions at APP. Therefore, we adopt a top-down optimization approach in which resource allocation at the MAC layer during the downloading of a chunk is constrained and guided by chunk bitrate from APP. This aims to align throughput closely with the chunk bitrate to maximize rate utilization. Assuming $e_{max}$ resource blocks are available at the base station, we formulate the integer linear programming problem for video-aware resource allocation (VRA) as:
\begin{equation*}
    \begin{aligned}
        &\rm \text{\textbf{P3:}} &&\underset{\{e_t\}_{t = 1,2,...,d_i}}{\rm \text{\textbf{min}}}
         \sum^{M_d}_{i=1}|\sum^{d_i}_{t = 1}N_{\tau_t, e_t}(1-\eta_{\gamma_t, e_t}) - \rho(a_{i,l})|\\
        &\rm \text{\textbf{s.t.}}
        & & \text{Constraints in Eqs. }  (1), (2), (5), (6). \\
        % & & & 0 \leq C_{\it{i+1}} \leq C^{\prime}_{\it{i}}, \\
    \end{aligned}
\end{equation*}
At time $t$ when decisions are made (at the start of each TTI), since the BLER is unknown, we utilizes Eq. (\ref{blerest}) to estimate BLER $\hat{\eta}_{\gamma_t, \tau_t}$ from past observations. The TB size $N_0$ that best matches the bitrate of the chunk is calculated as:
\begin{equation}
    N_{0} = \frac{\rho(a_{i,l})}{(1-\hat{\eta}_{\gamma_t, \tau_t})T_{\rm chunk}}.
\end{equation}
However, as the number of RBs is discrete, we cannot exactly transmit with TB size equal to $N_0$. Subsequently, we select $e_t$ from the set $\{0,1,...,e_{max}\}$, based on known MCS $\tau_t$ from soft link adaptation, whose TB size $N_{\tau_t, e_t}$ is closest to $N_0$. 




In order to integrate VRA into the allocation of resources for multiple users, the proportions of assigned RBs for each user with multi-user consideration are scaled by the ratio of RBs designated for a single user ($\frac{e_t}{e_{max}}$) as determined by our algorithm. Then, the ratio is normalized to determine the final distribution of resources among all users. Details of the resource allocation algorithm is shown in \textbf{Algorithm 2}. \par



\subsection{MAC: Video-aware Resource Allocation}
The MAC layer efficiently employs a scheduler to manage the allocation of RBs. The problem of MAC resource allocation is typically divided into two levels: multi-user and single-user. In multi-user allocation, the goal is to distribute resources fairly, usually by utilizing the waterfilling method or introducing proportional fairness. This distribution is then refined for individual users based on their specific task requirements. While we do not explore the multi-user allocation scenario, our proposed video-aware resource allocation (VRA) can be extended to the general multi-user case. 
Due to the longer time intervals (seconds) for bitrate decisions at the application layer compared to the shorter time slots (multiple of milliseconds) for resource allocation, it is challenging for lower-layer strategies to quickly impact the bitrate decisions at APP. Therefore, we suggest a top-down optimization approach in which resource allocation at the MAC layer during the download period of a chunk is constrained and guided by APP bitrate decisions. This approach aims to align transmission throughput closely with the chunk bitrate to maximize rate utilization. Assuming $e_{max}$ resource blocks are available at the base station, we formulate the integer linear programming problem for VRA as:
\begin{equation*}
    \begin{aligned}
        &\rm \text{\textbf{P3:}} &&\underset{\{e_t\}_{t = 1,2,...,d_i}}{\rm \text{\textbf{min}}}
         \sum^{M_d}_{i=1}|\sum^{d_i}_{t = 1}N_{\tau_t, e_t}(1-\eta_{\gamma_t, e_t}) - \rho(a_{i,l})|\\
        &\rm \text{\textbf{s.t.}}
        & & \text{Constraints in Eqs. }  (1), (2), (5), (6). \\
        % & & & 0 \leq C_{\it{i+1}} \leq C^{\prime}_{\it{i}}, \\
    \end{aligned}
\end{equation*}
At time $t$ when decisions are made (at the start of each TTI, which are multiples of slots), since BLER affects the throughput and changes with time, we utilizes Eq. (\ref{blerest}) to estimate BLER $\hat{\eta}_{\gamma_t, \tau_t}$. The TB size $N_0$ that best matches the bitrate of the chunk is calculated as:
\begin{equation}
    N_{0} = \frac{\rho(a_{i,l})}{(1-\hat{\eta}_{\gamma_t, \tau_t})T_{\rm chunk}}.
\end{equation}
Following this, we choose $e_t$ from the set $\{0,1,...,e_{max}\}$ using the selected MCS from soft link adaptation to adjust the TB size $N_{\tau_t, e_t}$ to be as near as possible to $N_0$. In order to integrate VRA into the allocation of resources for multiple users, the proportions of assigned RBs for each user with multi-user consideration are scaled by the ratio of RBs designated for a single user ($\frac{e_t}{e_{max}}$) as determined by our algorithm. Then, the ratio is normalized to determine the final distribution of resources among all users. Details of the resource allocation algorithm is shown in \textbf{Algorithm 2}. \par







